Disentangled Unsupervised Image Translation via Restricted Information Flow

Unsupervised image-to-image translation methods aim to map images from one domain into plausible examples from another domain while preserving structures shared across two domains. In the many-to-many setting, an additional guidance example from the target domain is used to determine domain-specific attributes of the generated image. In the absence of attribute annotations, methods have to infer which factors are specific to each domain from data during training. Many state-of-art methods hard-code the desired shared-vs-specific split into their architecture, severely restricting the scope of the problem. In this paper, we propose a new method that does not rely on such inductive architectural biases, and infers which attributes are domain-specific from data by constraining information flow through the network using translation honesty losses and a penalty on the capacity of domain-specific embedding. We show that the proposed method achieves consistently high manipulation accuracy across two synthetic and one natural dataset spanning a wide variety of domain-specific and shared attributes.

==> 1_intro_old.tex <==
\input{fig/problem}
\section{Introduction}
The goal of unsupervised many-to-many image translation is to turn an image from the source domain into an image from the target domain, preserving attributes shared between domains, and applying domain-specific attributes from a specified target image, also called ``a guide''. The model has no attribute supervision and has to infer which attributes vary in both domains and which variations are specific to each domain from two unlabeled sets of images. Figure \ref{fig:fig1_problem} illustrates that, for a source domain containing female faces with variable backgrounds, orientations, and hair colors, and a target domain containing images of brunette male faces with varied backgrounds, orientations, amount of facial hair, a successful method has to turn a female into a male, keeping the background textures and face orientations intact, and determining the amount of facial hair using a specified male guide image. The bottom section of Figure \ref{fig:fig1_problem} illustrates that attribute roles of same attributes might vary across different domain pairs: for front-facing children and middle-aged people on white backgrounds with variable face orientation, same attributes now have opposite roles: the hair color is shared, as it is varied in both domains, but backgrounds colors and face orientations only vary in respective domains, so both are domain-specific.

\input{fig/compare_shapes}
Prior work \cite{bashkirova2021evaluation} shows that existing methods generally fail to infer which attributes are shared or to manipulate them properly. More specifically, AdaIN-based methods~\cite{huang2018multimodal,choi2020stargan} inject domain-specific information from the guide image via a global feature re-normalization \cite{huang2017arbitrary}, forcing colors, textures, and other global statistics to be always treated as domain-specific factors regardless of their actual distribution across two domains. As a result, AdaIN-based methods change colors and textures of the input to match the guide image during translation even if these colors are varied across both domains. Autoencoder-based methods \cite{almahairi2018augmented,DRIT_plus,benaim2019didd}, on the other hand, preserve shared information better, but often fail to apply correct domain-specific factors. For example, Figure \ref{fig:shapes_compare} shows that the AdaIN-based method MUNIT \cite{huang2018multimodal} changes object color of the input to match the object color of the guide, even though object color is varied in both domains, and thus should be preserved, while autoencoder-based DIDD \cite{benaim2019didd} preserves the object color of the source, but fails to extract and apply the correct orientation and size from the guide. 
% A similar trend can be found on the brunette male-vs-female split of CelebA (Figure Y): MUNIT changes background color even though it is 
% Later, in Section X we show that the same happens on the CelebA split (Figure Y) - MUNIT treats backgrounds as domain-specific 
As a result, the majority of recently proposed best-performing unsupervised many-to-many translation methods use AdaIN, but assumptions hard-coded into this architecture choice severely restrict the kinds of problems that can be efficiently tackled
% using these methods 
to only those in which all colors, textures and backgrounds need not be preserved, which is often not the case, as illustrated in Figure~\ref{fig:fig1_problem}.

In this paper, we propose a novel approach that does not rely on an inductive bias provided by AdaIN and archives high attribute manipulation accuracy across different kinds of attributes regardless of whether they are shared or domain-specific. The core observation that lies in the heart of our method is that attributes that are shared across two domains can be ``represented naturally'' in the cross-domain translation result, while domain-specific attributes can only be  ``hidden'' in an image from another domain in the form of adversarial noise \cite{bashkirova2019adversarial}. More specifically, as illustrated in Figure~\ref{fig:method_overview}, to perform ``brunette male-to-female translation'' our method preserves \textit{shared factors} (background texture and orientation) of the input male face and encodes \textit{male-specific attributes} (mustache) in a side-channel embedding. In addition to well-established reconstruction (L1) and realism (GAN) losses, in this paper, we propose using the \textit{translation honesty} loss \cite{bashkirova2019adversarial} to penalize the model for ``hiding'' mustache inside the generated female image in the form of low-amplitude adversarial noise, and the \textit{embedding capacity} loss to penalize the model for using the side-channel embedding to encode background texture and orientation if it can encode them in the translation result. As a result, information about the mustache is pushed out of the translated image into the embedding, while information about the orientation and background is pushed out of the embedding into the translation result. We measure how well the proposed method manipulates different kinds of attributes as either shared or domain-specific across three splits of Shapes-3D~\cite{kim2018disentangling}, SynAction \cite{sun2020twostreamvan} and Celeb-A \cite{CelebAMask-HQ} following an evaluation protocol similar to the one proposed by \citet{bashkirova2021evaluation}. Our experiments confirm that the proposed method archives high attribute manipulation accuracy without relying on an inductive bias towards treating certain attribute kinds as domain-specific hard-coded into its architecture.

To summarize, in this paper we propose a new architecture for many-to-many image translation that uses translation honestly and channel capacity penalty, and does not rely on an inductive an bias provided by AdaIN, and show that, as a result, it achieves high attribute manipulation accuracy consistent across different combinations of shared and domain-specific attributes.

\input{fig/method_overivew}
\input{fig/table_overall}

==> fig/table_overall.tex <==
\begin{table}[t]\centering
% \small
% \inctabcolsep{-1pt} {
\inctabcolsep{-3pt} {
\begin{tabular}{lcccc} \toprule
\textbf{Method} & 3DS \cite{kim2018disentangling} & SA \cite{sun2020twostreamvan} & CA \cite{CelebAMask-HQ} & \textbf{AVG$\uparrow${\scriptsize$\pm\sigma$}} \\ \midrule
AugCycleGAN \cite{almahairi2018augmented} & 12 & 37 & 40 & 29{\scriptsize$\pm$15} \\
DIDD \cite{benaim2019didd} & 44 & 67 & \textbf{64} & 58{\scriptsize$\pm$12} \\
DRIT++ \cite{DRIT_plus} & 18 & 24 & 55 & 32{\scriptsize$\pm$20}\\
MUNIT \cite{huang2018multimodal} & \textit{58} & 37 & 53 & 49{\scriptsize$\pm$11} \\
MUNITX \cite{bashkirova2021evaluation} & 33 & 52 & 55 & 47{\scriptsize$\pm$12} \\
StarGANv2 \cite{choi2020stargan} & 45 & \textbf{82} & 51 & \textit{59{\scriptsize$\pm$20}} \\
RIFT (ours) & \textbf{66} & \textit{78} & \textit{60} & \textbf{68{\scriptsize$\pm$9}} \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Average attribute manipulation accuracy} across three splits of 3D-Shapes (3DS), a single split of SynAction (SA), and a single split of CelebA (CA). Our method achieves best or second-best performance across all three, and the best performance overall with lowest variance across datasets. {\color{red} I think this table should be swapped with figure 4.} \vspace{-10px}}\label{tab:overall}
\end{table}

==> fig/table_shapes_results.tex <==
\begin{table*}\centering
\begin{tabular}{lcccccccccccccc}\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{{FC}} & \multicolumn{2}{c}{{WC}} & \multicolumn{2}{c}{{OC}} & \multicolumn{2}{c}{{SZ}} & \multicolumn{2}{c}{{SH}} & \multicolumn{2}{c}{{ORI}} & \multicolumn{2}{c}{\textbf{AGG}} \\ \cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} \cmidrule(l){8-9} \cmidrule(l){10-11} \cmidrule(l){12-13} \cmidrule(l){14-15}
& S & D & S & D & S & D & S & D & S & D & S & D & {ACC}$\uparrow$ & {RD}$\downarrow$    \\
\midrule
StarGANv2 & 0 & 99 & 0 & 99 & 0 & 78 & 5 & 56 & 4 & 99 & 0 & 96 & 45 & 97 \\
% StarGANv2 & 0 & 95 & 0 & 95 & 5 & 78 & 5 & 36 & 11 & 99 & 0 & 50 & 46 & 98 \\
MUNIT & 5 & 94 & 0 & 99 & 0 & 97 & 59 & 31 & 96 & 58 & 99 & 61 & 58 & 56 \\
MUNITX & 1 & 50 & 2 & 55 & 8 & 28 & 12 & 16 & 95 & 21 & 99 & 7 & 33 & 74 \\
DRIT & 7 & 12 & 9 & 19 & 10 & 10 & 27 & 14 & 7 & 15 & 42 & 51 & 18 & \textbf{20} \\
AugCycleGAN & 10 & 8 & 10 & 9 & 11 & 7 & 17 & 13 & 30 & 13 & 7 & 7 & 12 & \textbf{20} \\
DIDD & 38 & 81 & 29 & 22 & 72 & 18 & 41 & 20 & 87 & 43 & 48 & 34 & 44 & 35 \\
Ours & 99 & 45 & 99 & 39 & 92 & 10 & 50 & 23 & 62 & 84 & 98 & 87 & \textbf{66} & 33 \\
\midrule
RAND & 10 & 10 & 10 & 10 & 10 & 10 & 12 & 19 & 24 & 19 & 6 & 6 & 12 & 9 \\
\bottomrule
\end{tabular}
\caption{\textbf{Manipulation accuracy} aggregated across different splits of \textbf{Shapes-3D} described in Section~\ref{sec:experiment} and illustrated in Figure~\ref{fig:shapes_examples}. For each of six attributes: color (FC), wall color (WC), object color (OC), size (SZ), shape (SH), room orientation (ORI) - we report \textit{aggregated manipulation accuracies} for when that attribute is shared (S) or domain-specific (D). We also report overall \textit{average aggregated manipulation accuracy} as well as \textit{relative discrepancy} between the accuracy of manipulating each attribute as domain-specific or shared. A Table~\todo{?} with non-aggregated performance across three splits can be found in supplementary. }
\label{tab:shape_results}
\end{table*}

==> fig/table_synaction.tex <==
\begin{table*}\centering
\begin{tabular}{lccccccccccc}\toprule
& \multicolumn{4}{c}{SynAction \cite{sun2020twostreamvan}} & \multicolumn{7}{c}{CelebA \cite{CelebAMask-HQ} } \\
\cmidrule(lr){2-5} \cmidrule(lr){6-12}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{PS} & \multicolumn{1}{l}{IDT} & \multicolumn{1}{l}{BG} & \multicolumn{1}{l}{\textbf{AVG}$\uparrow$} & HC & FH & GD & ORI & BG & SC & \textbf{AVG}$\uparrow$ \\ 
& S & D & D & - & D & D & D & S & S & S & - \\
\midrule
StarGANv2 & \textbf{96} & \textbf{52} & \textbf{99} & \textbf{82} & \textbf{76} & 15 & 97 & 87 & 11 & 22 & 51 \\
MUNIT & 75 & 28 & 7 & 37 & 45 & 7 & 90 & \textbf{89} & 43 & 44 & 53 \\
MUNITX & 93 & 26 & 37 & 52 & 64 & 17 & 75 & 83 & 50 & 43 & 55 \\
DRIT & 52 & 6 & 13 & 24 & 23 & 9 & 96 & \textbf{89} & 67 & 44 & 55 \\
AugCycleGAN & 90 & 8 & 12 & 37  & 16 & 30 & 98 & 12 & 42 & 40 & 40 \\
DIDD & 89 & 12 & \textbf{99} & 67 & 22 & \textbf{50} & 91 & 78 & \textbf{89} & 56 & \textbf{64} \\ 
Ours & 89 & 47 & \textbf{99} & 78 & 22 & 35 & \textbf{99} & 65 & 83 & \textbf{57} & 60 \\ \midrule
RAND & 50 & 11 & 11 & 24 & \todo{?} & \todo{?} & \todo{?} & \todo{?} & \todo{?} & \todo{?} & \todo{?} \\ \bottomrule
\end{tabular}
\caption{ }
\end{table*}

==> kate-intro.tex <==
\input{fig/problem}

\section{Introduction}

Unsupervised image-to-image translation learns a mapping between two sets of images or two ``domains". A good translation method must learn which attributes are shared across domains and should thus be preserved, and which attributes only appear in one domain and should thus be changed. For example, the domains in Fig.~\ref{fig:fig1_problem}(b) share the pose attribute but gender is domain-specific, so the mapping must preserve the original pose but change the gender. When a domain has multiple unique attributes, like males with beards and males without beards, the mapping becomes many-to-many. The method is then given an additional input ``guide" image (Fig.~\ref{fig:fig1_problem}(a)) from which it must infer the correct domain-specific attribute(s) to use.

State-of-the-art methods for unsupervised many-to-many translation assume that the domain-specific variations can be modeled as ``global style" (textures and colors) and hard-code this assumption into their architectures. However, this choice severely restricts the kinds of problems that can be efficiently solved, as illustrated in Figure~\ref{fig:fig1_problem}(c). In this example the domains are children vs. adults where the hair color is shared by both domains and should be preserved, but face pose only varies in the adults domain and should be changed. 
Existing methods generally fail to infer and manipulate such  domain-specific attributes unrelated to global style correctly, as was recently shown by \cite{bashkirova2021evaluation}

\input{fig/compare_shapes}
More specifically, AdaIN-based methods~\cite{huang2018multimodal,choi2020stargan} inject domain-specific information from the guide image via a global feature re-normalization \cite{huang2017arbitrary} which forces colors, textures, and other global statistics to be always treated as domain-specific factors regardless of their actual distribution across the two domains. As a result, AdaIN-based methods change colors and textures of the input to match the guide image during translation even if colors/textures are varied across both domains and should not change. Autoencoder-based methods \cite{almahairi2018augmented,DRIT_plus,benaim2019didd}, on the other hand, preserve shared information better, but often fail to apply correct domain-specific factors. For example, Fig.~\ref{fig:shapes_compare} shows that the AdaIN-based method MUNIT \cite{huang2018multimodal} changes object color of the input to match the object color of the guide, even though object color is varied in both domains, and thus should be preserved. The autoencoder-based DIDD \cite{benaim2019didd} preserves the object color of the source, but fails to extract and apply the correct orientation and size from the guide. 

In this paper, we propose a novel approach that does not rely on an inductive bias provided by AdaIN and achieves high attribute manipulation accuracy across different kinds of attributes regardless of whether they are shared or domain-specific. The core observation at the heart of our method is that attributes that are shared across two domains can be represented naturally in the cross-domain translation result, while domain-specific attributes can only be hidden in an image from another domain in the form of adversarial noise \cite{bashkirova2019adversarial}. More specifically, as illustrated in Figure~\ref{fig:method_overview}, to perform ``brunette male-to-female translation'' our method preserves \textit{shared factors} (background texture and orientation) of the input male face and encodes \textit{male-specific attributes} (mustache) in a side-channel embedding. In addition to well-established reconstruction (L1) and realism (GAN) losses, in this paper, we propose using the \textit{translation honesty} loss \cite{bashkirova2019adversarial} to penalize the model for ``hiding'' mustache inside the generated female image in the form of low-amplitude adversarial noise, and the \textit{embedding capacity} loss to penalize the model for using the side-channel embedding to encode background texture and orientation if it can encode them in the translation result. As a result, information about the mustache is pushed out of the translated image into the embedding, while information about the orientation and background is pushed out of the embedding into the translation result. 

We measure how well the proposed method models different kinds of attributes as either shared or domain-specific across three splits of Shapes-3D~\cite{kim2018disentangling}, SynAction \cite{sun2020twostreamvan} and Celeb-A \cite{CelebAMask-HQ} following an evaluation protocol similar to the one proposed by \citet{bashkirova2021evaluation}. Our experiments confirm that the proposed method archives high attribute manipulation accuracy without relying on an inductive bias towards treating certain attribute kinds as domain-specific hard-coded into its architecture.


\input{fig/method_overivew}
